Are LLMs Good Annotators for Discourse-level Event Relation Extraction?

Large Language Models (LLMs) have demonstrated proficiency in a wide array of natural language processing tasks. However, its effectiveness over discourse-level event relation extraction (ERE) tasks remains unexplored. In this paper, we assess the effectiveness of LLMs in addressing discourse-level ERE tasks characterized by lengthy documents and intricate relations encompassing coreference, temporal, causal, and subevent types. Evaluation is conducted using an commercial model, GPT-3.5, and an open-source model, LLaMA-2. Our study reveals a notable underperformance of LLMs compared to the baseline established through supervised learning. Although Supervised Fine-Tuning (SFT) can improve LLMs performance, it does not scale well compared to the smaller supervised baseline model. Our quantitative and qualitative analysis shows that LLMs have several weaknesses when applied for extracting event relations, including a tendency to fabricate event mentions, and failures to capture transitivity rules among relations, detect long distance relations, or comprehend contexts with dense event mentions. Code available at: https://github.com/WeiKangda/LLM-ERE.git.

==> coreference_table_valid.tex <==
\begin{table*}[t!]
\small
% \normalsize
%\scriptsize
\footnotesize
%\tiny
\begin{center}
\scalebox{0.9}{\begin{tabular}{ lrrr|rrr|rrr|rrr} 
 \toprule
& \multicolumn{3}{c|}{\textbf{MUC}} & \multicolumn{3}{c|}{\textbf{B^{3}}} & \multicolumn{3}{c|}{\textbf{CEAF_{e}}} & \multicolumn{3}{c}{\textbf{BLANC}} \\
 
\textbf{\textbf{Prompt}} & Precision & Recall & F-1 & Precision & Recall & F-1 & Precision & Recall & F-1 & Precision & Recall & F-1\\

 \midrule
 Bulk prediction \ruihong{Is this zero-shot result?} & $3.3$ & $14.3$ & $5.3$ & $77.7$ & $95.1$ & $85.5$ & $87.4$ & $71.0$ & $78.3$ & $51.4$ & $53.6$ & $51.9$\\
 \midrule
 Whole doc & $9.5$ & $28.6$ & $14.3$ & $85.3$ & $95.8$ & $90.1$ & $92.8$ & $82.4$ & $87.3$ & $52.6$ & $59.8$ & $53.8$\\ 
 1-shot & $2.4$ & $7.1$ & $3.6$ & $84.6$ & $94.9$ & $89.4$ & $91.9$ & $82.0$ & $86.6$ & $50.2$ & $50.9$ & $50.0$\\ 
 2-shot & $\mathbf{10.6}$ & $\mathbf{35.7}$ & $\mathbf{16.4}$ & $83.2$ & $\mathbf{96.0}$ & $89.2$ & $93.0$ & $80.8$ & $86.5$ & $52.3$ & $61.6$ & $53.4$\\ 
 5-shot & $7.7$ & $21.4$ & $11.3$ & $\mathbf{86.0}$ & $95.6$ & $\mathbf{90.5}$ & $92.5$ & $83.2$ & $87.6$ & $\mathbf{52.9}$ & $\mathbf{61.9}$ & $\mathbf{54.3}$\\ 
 10-shot & $5.1$ & $14.3$ & $7.6$ & $85.8$ & $95.3$ & $90.3$ & $\mathbf{93.2}$ & $\mathbf{83.9}$ & $\mathbf{88.3}$ & $50.9$ & $53.3$ & $51.2$\\
 \midrule
 Event ranking & $4.4$ & $14.3$ & $6.7$ & $83.3$ & $95.1$ & $88.8$ & $88.9$ & $77.5$ & $82.8$ & $51.9$ & $53.8$ & $52.5$\\
\bottomrule

\end{tabular}}
\end{center}
\caption{Event coreference performances of \textit{gpt-3.5-turbo-16k} on \mavenere using different prompt patterns one the first 10 documents of the validation set. The numbers in \textbf{bold} indicate the best performance across different prompt patterns for \textit{gpt-3.5-turbo-16k}.}
\vspace{-0.1in}
\label{tab:coreference-table-valid}
\end{table*}

==> distance_error_analysis_sentence_table.tex <==
\begin{table}[htb]
\small
% \normalsize
%\scriptsize
\footnotesize
%\tiny
\begin{center}
\scalebox{0.75}{\begin{tabular}{l | c c c c c c c}
    \midrule
     & & $<1$ & $1$ & $2$ & $3$ & $4$ & $>=5$\\
     %\midrule
     %\multirow{3}{*}{whole doc} & Temporal & $18.18$ & $15.60$ & $12.21$ & $5.60$ & $7.05$ &$8.80$\\
     %& Causal & $6.15$ & $0$ & $5.63$ & $5.56$ & $0$& $0$\\
     %& Subevent & $0$ & $3.57$ & $6.25$ & $13.33$ & $0$ & $0$\\
     \midrule
     \multirow{3}{*}{10-shot} & Temporal & $25.45$ & $19.97$ & $17.70$ & $10.23$ & $11.76$ & $6.87$\\
     &Causal & $8.92$ & $11.02$ & $7.69$ & $0$ & $0$ & $8.70$\\
     &Subevent & $4.65$ & $5.26$ & $0$ & $0$ & $0$ & $0$\\
     \midrule
\end{tabular}}
\end{center}
\vspace{-0.1in}
\caption{GPT-3.5 performance (F-1 score) using Iterative Prediction 10-shot prompt on data groups with different distances (measured in \#sentences) between related events of different relation types.}
\vspace{-0.1in}
\label{tab:distance_error_analysis_sentence_table}
\end{table}

==> distance_error_analysis_table.tex <==
\begin{table}[htb]
\small
% \normalsize
%\scriptsize
\footnotesize
%\tiny
% \begin{center}
\scalebox{1.0}{\begin{tabular}{l | c c c c}
    \midrule
     & &$<50$ & $50-200$ & $>200$\\
     \midrule
     \multirow{3}{*}{whole doc} & Temporal & $15.54$ & $9.71$ & $9.55$ \\
     &Causal & $3.39$ & $2.45$ & $0$ \\
     &Subevent & $3.67$ & $3.13$ & $0$ \\
     \midrule
     \multirow{3}{*}{10-shot} & Temporal & $21.17$ & $10.56$ & $8.29$ \\
     &Causal & $8.78$ & $4.65$ & $11.76$ \\
     &Subevent & $4.62$ & $0$ & $0$ \\
     \midrule
\end{tabular}}
% \end{center}
\vspace{-0.1in}
\caption{GPT-3.5 performance (F-1 score) using Iterative Prediction whole doc and 10-shot prompt on data groups with different distances (measured in \#tokens ) between related events of different relation types.}
\vspace{-0.1in}
\label{tab:distance_error_analysis_table}
\end{table}

==> inter_intra_sentence.tex <==
\begin{table}[htb]
\small
% \normalsize
%\scriptsize
\footnotesize
%\tiny
\begin{center}
    \scalebox{0.9}{\begin{tabular}{l | c c c }
    \midrule
     & & Intra & Inter\\
     \midrule
     \multirow{3}{*}{10-shot} & Temporal & $25.45$ & $12.39$\\
     &Causal & $8.92$ & $7.02$\\
     &Subevent & $4.65$ & $2.56$\\
     \midrule
\end{tabular}}
\end{center}
\vspace{-0.1in}
\caption{GPT-3.5 performance (F-1 score) using Iterative Prediction 10-shot prompt on event pairs inter- and intra-sentence of different relation types.}
\vspace{-0.1in}
\label{tab:inter_intra_table}
\end{table}

==> query_number.tex <==
\begin{table}[htb]
\small
% \normalsize
%\scriptsize
%\footnotesize
%\tiny
\begin{center}
\scalebox{1.0}{\begin{tabular}{c c c}
    \midrule
     & \# of queries & Overall F-1\\
     \midrule
     Bulk Prediction & $4$ & $16.5$ \\
     Iterative Prediction & $45$ & $21.2$ \\
     Event Ranking & $240$ & $22.7$ \\
     \midrule
\end{tabular}}
\end{center}
\vspace{-0.1in}
\caption{Average number of queries needed for one document using Bulk Prediction, Iterative Prediction, and Event Ranking}
\vspace{-0.1in}
\label{tab:query-number-table}
\end{table}

==> rest_table.tex <==
\begin{table}[t!]
\small
% \normalsize
%\scriptsize
\footnotesize
%\tiny
\begin{center}
\scalebox{0.95}{\begin{tabular}{ l|cccc} 
 \toprule
 Relation & \begin{tabular}[c]{@{}c@{}}Iterative\\Prediction\end{tabular} & Precision & Recall & F-1\\
 \midrule
 \multirow{6}{*}{Temporal} & whole doc & $19.8$ & $4.4$ & $7.2$ \\ 
 & 1-shot & $17.1$ & $4.5$ & $7.1$\\ 
 &2-shot & $19.5$ & $4.3$ & $7.1$ \\ 
 &5-shot & $21.3$ & $5.8$ & $9.1$ \\ 
 &10-shot & $\mathbf{26.8}$ & $\mathbf{8.0}$ & $\mathbf{12.3}$ \\
 \cmidrule{2-5} &Baseline & $57.3_{0.6}$ & $54.5_{0.1}$ & $55.8_{0.2}$\\
 \midrule
 \multirow{6}{*}{Causal} & whole doc & $2.9$ & $2.9$ & $2.8$ \\ 
 & 1-shot & $4.1$ & $2.7$ & $3.3$\\ 
 &2-shot & $4.1$ & $2.6$ & $3.2$ \\ 
 &5-shot & $4.5$ & $3.0$ & $3.6$ \\ 
 &10-shot & $\mathbf{5.3}$ & $\mathbf{5.3}$ & $\mathbf{5.3}$ \\
 \cmidrule{2-5} &Baseline & $34.2_{0.1}$ & $29.3_{1.0}$ & $31.6_{0.6}$\\
 \midrule
 \multirow{6}{*}{Subevent} & whole doc & $\mathbf{1.9}$ & $1.3$ & $1.6$ \\ 
 & 1-shot & $1.9$ & $1.2$ & $1.5$\\ 
 &2-shot & $1.5$ & $0.9$ & $1.2$ \\ 
 &5-shot & $1.7$ & $1.4$ & $1.6$ \\ 
 &10-shot & $1.7$ & $\mathbf{2.8}$ & $\mathbf{2.1}$ \\
 \cmidrule{2-5} & Baseline & $29.5_{2.5}$ & $25.4_{2.6}$ & $27.2_{0.9}$\\
\bottomrule
\end{tabular}}
\end{center}
\vspace{-0.1in}
\caption{Performance of GPT-3.5 for extracting temporal, causal, and subevent relations on \mavenere test set using Iterative prediction prompts. \textbf{Bold} denotes the best performance among different prompt patterns. We report averages and standard deviations over 3 random seeds for the baseline method.}
%\vspace{-0.5cm}
\label{tab:rest-table}
\end{table}

==> rest_table_llama.tex <==
\begin{table}[t!]
\small
% \normalsize
%\scriptsize
\footnotesize
%\tiny
\begin{center}
\scalebox{0.95}{\begin{tabular}{ l|cccc} 
 \toprule
 Relation & \begin{tabular}[c]{@{}c@{}}Iterative\\Prediction\end{tabular} & Precision & Recall & F-1\\
 \midrule
 \multirow{6}{*}{Temporal} & whole doc & $17.2$ & $\mathbf{3.1}$ & $\mathbf{5.2}$ \\ 
 & 1-shot & $15.4$ & $1.2$ & $2.2$\\ 
 &2-shot & $\mathbf{26.3}$ & $2.2$ & $4.1$ \\ 
 &5-shot & $19.4$ & $1.3$ & $2.4$ \\ 
 \cmidrule{2-5} &Baseline & $57.3_{0.6}$ & $54.5_{0.1}$ & $55.8_{0.2}$\\
 \midrule
 \multirow{6}{*}{Causal} & whole doc & $4.1$ & $\mathbf{5.0}$ & $\mathbf{4.5}$ \\ 
 & 1-shot & $4.6$ & $0.2$ & $0.3$\\ 
 & 2-shot & $4.6$ & $0.1$ & $0.2$ \\ 
 & 5-shot & $\mathbf{8.2}$ & $0.2$ & $0.3$ \\ 
 \cmidrule{2-5} &Baseline & $34.2_{0.1}$ & $29.3_{1.0}$ & $31.6_{0.6}$\\
 \midrule
 \multirow{6}{*}{Subevent} & whole doc & $3.4$ & $\mathbf{6.3}$ & $\mathbf{4.4}$ \\ 
 & 1-shot & $3.3$ & $0.1$ & $0.2$\\ 
 &2-shot & $0$ & $0$ & $0$ \\ 
 &5-shot & $\mathbf{4.5}$ & $0.2$ & $0.4$ \\ 
 \cmidrule{2-5} & Baseline & $29.5_{2.5}$ & $25.4_{2.6}$ & $27.2_{0.9}$\\
\bottomrule
\end{tabular}}
\end{center}
\vspace{-0.1in}
\caption{Performance of LLaMA-2 for extracting temporal, causal, and subevent relations on \mavenere test set using Iterative prediction prompts. \textbf{Bold} denotes the best performance among different prompt patterns. We report averages and standard deviations over 3 random seeds for the baseline method.}
%\vspace{-0.5cm}
\label{tab:rest-table-llama}
\end{table}

==> rest_table_valid.tex <==
\begin{table}[t!]
\small
% \normalsize
%\scriptsize
\footnotesize
%\tiny
\begin{center}
\scalebox{0.95}{\begin{tabular}{ l|cccc} 
 \toprule
 Relation & Prompt & Precision & Recall & F-1\\
 \midrule
 \multirow{6}{*}{Temporal} & Bulk prediction & $7.2$ & $2.3$ & $3.4$ \\
 \cmidrule{2-5} & Whole doc & $19.9$ & $8.6$ & $11.2$ \\ 
 & 1-shot & $18.0$ & $10.4$ & $13.2$\\ 
 &2-shot & $18.5$ & $7.1$ & $10.2$ \\ 
 &5-shot & $16.3$ & $8.0$ & $10.8$ \\ 
 &10-shot & $\mathbf{22.1}$ & $10.6$ & $14.3$ \\
 \cmidrule{2-5} & Event ranking & $15.8$ & $\mathbf{34.1}$ & $\mathbf{21.6}$\\
 \midrule
 \multirow{6}{*}{Causal} & Bulk prediction & $2.8$ & $2.4$ & $2.6$ \\
 \cmidrule{2-5} & Whole doc & $2.2$ & $4.2$ & $2.9$ \\ 
 & 1-shot & $5.0$ & $7.7$ & $6.1$\\ 
 &2-shot & $4.6$ & $6.0$ & $5.2$ \\ 
 &5-shot & $3.9$ & $4.8$ & $4.3$ \\ 
 &10-shot & $\mathbf{6.2}$ & $\mathbf{10.1}$ & $\mathbf{7.7}$ \\
 \cmidrule{2-5} &Event ranking & $4.8$ & $7.6$ & $5.9$\\
 \midrule
 \multirow{6}{*}{Subevent} & Bulk prediction & $3.0$ & $\mathbf{9.8}$ & $4.6$ \\
 \cmidrule{2-5} & Whole doc & $2.1$ & $7.3$ & $3.3$ \\ 
 & 1-shot & $2.8$ & $\mathbf{9.8}$ & $4.3$\\ 
 &2-shot & $3.2$ & $7.3$ & $4.4$ \\ 
 &5-shot & $0.0$ & $0.0$ & $0.0$ \\ 
 &10-shot & $2.0$ & $\mathbf{9.8}$ & $3.3$ \\
 \cmidrule{2-5} & Event ranking & $\mathbf{4.4}$ & $7.9$ & $\mathbf{5.7}$\\
\bottomrule
\end{tabular}}
\end{center}
\caption{Performance of \textit{gpt-3.5-turbo-16k} for extracting temporal, causal, and subevent relations on the first 10 validation documents of \mavenere. \textbf{Bold} denotes the best performance among different prompt patterns.}
\vspace{-0.5cm}
\label{tab:rest-table-valid}
\end{table}
